An Information Centric Framework for Weather Sensing Data

Weather sensing and forecasting has become increasingly accurate in the last decade thanks to high-resolution radars, efficient computational algorithms, and high-performance computing facilities. Through a distributed and federated network of radars, scientists can make high-resolution observations of the weather conditions on a scale that benefits public safety, commerce, transportation, and other fields. While weather radars are critical infrastructure, they are often located in remote areas with poor network connectivity. Data retrieved from these radars are often delayed or lost, or even lack proper synchronization, resulting in sub-optimal weather prediction. This work applies Named Data Networking (NDN) to a federation of weather sensing radars for efficient content addressing and retrieval. We identify weather data based on a hierarchical naming scheme that allows us to explicitly access desired files. We demonstrate that compared to the window-based mechanism in TCP/IP, an NDN based mechanism improves data quality, reduces uncertainty, and enhances weather prediction. Our evaluation demonstrates that this naming scheme enables effective data retrieval, while compared to the window-based mechanism in TCP/IP, an NDN based mechanism improves data quality, reduces uncertainty, and enhances weather prediction.

==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}



\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
%\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
%\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> old-2-background.tex <==
\section{Background}
\label{sec:background}
\subsection{CASA}
\label{subsec:casa}
% The NSF Engineering Research Center for Collaborative Adaptive Sensing of the Atmosphere 
CASA was formed to study the lower atmosphere with networks of high resolution Doppler weather radars with the goal to improve severe weather awareness \cite{MPC+09}. The volumetric data produced by these continuously operating remote sensors must be distributed to processing servers quickly and efficiently, such that analysis can occur in near real time for the sake of warning the public to fast developing threats such as tornadoes and high winds. The networked radar concept requires that asynchronous raw data from multiple sources is blended together to create value-added meteorological products. At any given time the characteristics of the ongoing weather regime determine the necessity and priority of certain products. For example, a hail detection algorithm takes on high importance only when strong thunderstorms are ongoing, whereas forecasting algorithms may be of more importance well in advance of such severe weather events and perhaps somewhat less so once the event has started.

Currently, CASA operates a network of seven X-band radars in the Dallas/Fort Worth (DFW) Metroplex~\cite{casadfw}. These radars have mechanically steered antennas and are tasked to perform surveillance scans (antenna rotates a full 360$^\circ$) at different elevation angles. Since the radars are not identical their form of producing atmospheric data is slightly different, and data generation is not synchronized across all radars (e.g., the execution of a surveillance scan does not take the same amount of time for all radars). In Section~\ref{subsubsec:dataflow}, we provide an overview of the current data flow paradigm and Sect.~\ref{subsubsec:asyncdata} outlines the challenges related to this approach and motivates how Information Centric Networking can mitigate these challenges.
%\todo{Add Figure of radar network?}

\subsubsection{Current Dataflow Paradigm}
\label{subsubsec:dataflow}
The underlying data transport mechanisms used in the CASA network are based on the traditional TCP/IP protocol stack. For example, UCAR's Local Data Manager (LDM) system~\cite{unidataldm} is used for event based distribution and analysis of radar data. The event based distribution relies on a sender-driven pub/sub system, whereby data requests from downstream clients are registered with regex-like pattern match schemes based on expected file naming conventions.  Data filenames generally include product or radar name, valid time, and the file format abbreviation as suffix.  Client side data requests include the IP address or DNS name of the upstream server associated with each product pattern and these are contained in a configuration file.  The upstream data server must include a corresponding configuration entry allowing the downstream client IP address/DNS name to request such data.  Any changes to the configuration files on either client or server side require a program restart to take effect, during which all data ceases to flow for several seconds. Thereafter, any data arriving to or input from the server side matching the client's requested pattern is forwarded to the client.  Data flows and the applications using the data are disjointed in this respect.  This sender-driven approach is not well suited for mostly-data driven algorithms since a priori knowledge of active algorithms and their data needs is required, and modifications to the data retrieval service is disruptive to the overall system and potentially other users. %In addition,
The paradigm of preconfigured data retrieval on a per machine basis is not well suited for the virtualized, cloud-based, highly adaptive compute resource that are used in the CASA system today~\cite{escience2019}. The current CASA data processing architecture and potential future generations will benefit from an approach that allows applications to pull data as they are needed. This approach will eliminate the need for a priori knowledge of the applications compute resource and data requirements.
\begin{comment}
Dynamic product creation on scarce compute resources is not well suited to the paradigm of preconfigured data retrieval on a per machine basis.  Future processing systems may benefit by allowing applications to pull data as it is needed, removing the need for a priori knowledge of the applications and data requirements that may be running at a given time.
\end{comment}
%\todo{do we make this comment visible?}

\subsubsection{Asynchronous Data}
\label{subsubsec:asyncdata}
% The CASA radar network is composed of a heterogeneous set of sensors (weather radars) with different update rates, scanning strategies, time and spatial resolutions, data sizes, and access network infrastructure.  
The operation of the radars in the CASA network is not synchronized in any respect, however the data they generate still needs to be mosaicked at a central processing location, and there is still a notion of an ideal set of data files that should be ingested for each mosaic.  In general, a mosaic is a full volumetric set of data from each radar, as closely linked in time as possible.  Radars produce volumes made up of multiple data files at intervals from 50 to 70 seconds.  It is less than ideal to not include some of the data files making up a volume in the mosaicking process, but also less than ideal to include data files representing the same portion of the volume at multiple times, which results in a smearing effect. Time based windowing, whereby an algorithm waits for a specified period of time for data from all radars to arrive, then executes based on the input it received quite often leads to one or the other of these results. Moreover a result we always strive to avoid is to not include any data from a radar in a mosaic, starving regions of the grid of all data and possibly causing users to make ill informed decisions.  Therefore the time windows must be kept open longer than the ideal interval, so as to guarantee in all normal  network traffic situations that at least one file from each radar shall arrive and be included in the mosaic.  A better solution would be to request all data files making up a volume from each radar in an explicit fashion. Current time-based naming schemes can make this problematic to request, so we propose an alternative scheme indicative of the periodic volumetric collections of data files from each radar and explained in detail in Section~\ref{subsec:scheme}.

\subsection{NDN}
\label{subsec:ndn}
Named Data Networking (NDN)~\cite{Zhang:NDN:CCR2014} has gained traction in recent years due to its hop-by-hop connectivity based on content instead of finite address-based communication amongst hosts. This new approach of using uniquely named content as the core internet principle makes communication independent of location, application, and means of transportation.
%Named Data Networking, abbreviated as NDN, is one such specific ICN architecture design. 
Even though it represents an entirely new architecture, NDN preserves the internet's hourglass architecture, making it compatible to run over and along with existing IP. NDN is particularly beneficial while considering large-scale data dissemination instead of IP that faces challenges when it comes to fixed point-to-point data delivery. %Moreover, NDN's automatic in-network caching imposes a huge advantage over IP when dealing with a large amount of data.\\
NDN communication has two components: \textit{Interest} and \textit{Data} packets. Interest packets are requests for content sent by a consumer to fetch a data packet generated by the producer in return. All the communication is secure as all the data packets are signed. Each NDN node has a stateful forwarding plane that consists of a Content Store (CS), a Pending Interest Table (PIT), and a Forwarding Strategy that includes the Forwarding Information Base (FIB). %The FIB has the forwarding strategy rules required for routing, and PIT is the table that stores incoming \textit{Interest} details. When an \textit{Interest} arrives and matches a PIT entry, the incoming interface info is added to the PIT table. 
If the  \textit{Data} for an \textit{Interest} packet has been served before, it would have been stored in the CS and directly served from the cache. On no match on either of these tables, the FIB table is referred for routing the packet.

Additionally, NDN uses a pull based model rather than IP's push based model. This gives the control of content retrieval to the consumer rather than the producer. Consequently, consumers can decide when and how to retrieve content from the producer. Additionally, in-network caches lead to better scalability, robustness, and faster failure recovery.

% Spyros added that
\subsection{Why not use TCP/IP?}
In federated networks of radars, the radars may communicate with clients through paths consisting of several network hops. These paths may span different service providers, become congested over time, have certain bandwidth constraints, while the overall connectivity between radars and clients may be intermittent. TCP/IP relies on end-to-end connections, without any support from the network infrastructure. However, in NDN, the network can utilize multiple available paths in parallel, adapt to network failures, and facilitate fast retransmissions. At the same time, solutions, such as SSL/TLS, which are widely used in TCP/IP, secure the communication channels, largely depending on the underlying connectivity. On the other hand, NDN makes security a property of the data itself, decoupling it from the underlying connectivity.


\subsection{Why not use HTTP?}

Similarly, we could create similar functionality using HTTP(s). However, HTTP relies on underlying IP infrastructure and inherits the problems we discussed above. While HTTP allows us to retrieve data based on names, it does not provide robustness against network congestion or failure. Since paths are end-to-end, HTTP is not able to switch routes even when multiple (potentially less congested) routes are available. Finally, unlike NDN, HTTP is unable to provide fast retransmission after packet loss since the packet caches are at the application layer. Finally, in this scenario, where we expect to see some packet loss due to the remote location of the radars. HTTP may not work well in this scenario.

==> old-3-relatedwork.tex <==
\section{Related Work}
\label{sec:relwork}

\subsection{Weather Sensing}
\label{subsec:rwcasa}
In contrast to the nationwide NEXRAD radar network operated by the National Weather Service (NWS) which consists of 160 homogeneous radars, the CASA system in DFW consists of a heterogeneous and federated network of radars. 

While in the NEXRAD system there is only little atmospheric volume that is covered by more than one radar, a significant portion of the coverage area of the CASA system is covered by 2 (or in some cases 3) radars. Thus, merging the individual radar data in a mosaic in a timely manner is important for algorithms that use these merged data for weather product generation.

Current radar networks (including NEXRAD) make use of data distribution applications like LDM~\cite{unidataldm} that are implemented on top of the traditional TCP/IP stack. Contrary, the work presented in this paper presents a new approach based on NDN to make radar data distribution and the execution of weather algorithms more efficient. Zhang et al.~\cite{Zhang:Infocom:2017} have presented a synchronization protocol that is also designed for the distribution of weather data. While the work presented by Zhang et al. focuses on the distribution of weather products to the end users, our approach focuses on the generation of such products by providing a new approach for transmitting data from the radars to a central compute site where weather product algorithms are running. In addition, our design and proposed naming scheme for data generation and retrieval in rounds is inspired by RoundSync, a protocol for distributed dataset synchronization in NDN~\cite{de2017design}.


\subsection{Named Data Networking}
\label{subsec:relndn}


Distributed science use cases naturally fit into NDN's name based paradigm. NDN's naming paradigm fits nicely with the existing naming conventions since NDN only encourages the name structures to be hierarchical and names to be human-readable and semantically meaningful providing some additional level of assurance.

We have shown in our previous work~\cite{olschanowsky2014supporting} that using a name-based system to publish, discover, and retrieve these distributed large datasets can reduce data management complexity ~\cite{shannigrahi2015named, fan2015managing} and speed up content delivery. Additionally, we found that these communities either utilize hierarchical and semantically meaningful names or these names are easily translatable into NDN names~\cite{shannigrahi2020s}.  

%For example, we found that a number of climate community uses data names that can be generalized as  \texttt{/Activity/[Sub-Activity or Product]/Organization/Model/<data specific components>}. One such name might look like \ndnName{/CMIP5/output/MIROC/MIROC4h/historical/6hr/atmos/psl/r1i1p1/1950010100-1950013100/}. The name tells the user some details about the data  (that it contains historical sea level atmospheric pressure data over the given time period). This naming scheme not only provides the necessary information to the user but also allows an NDN network to forward Interests and Data packets based on these names.% A CMIP5 data repository (or repositories) can simply announce /CMIP5 into the network. The NDN network then forwards any Interest beginning with /CMIP5 to the data source. If data is replicated and available from multiple repositories, the network decides the ``best" data source. In our experience, similar name based data organization is possible in high energy particle physics \cite{shannigrahi2015named}, genomics \cite{shannigrahi2018named}, and other scientific communities. Naming data hierarchically and utilizing those names in an NDN network not only speeds up content delivery but also reduces network load as well as application complexity. 

In this work we create a similar hierarchical naming scheme -  \ndnName{/radarName/round/sequence/} (see \ref{subsec:rounds} for details). The naming scheme captures essential information (radar location, rotational information such as round and sequence number) and allows us to efficiently retrieve data over the network for the workflow. The hierarchical naming scheme also allows for future expansion - we might add timestamp and some location information depending on the workflow.


